Staleness-aware Async-SGD for Distributed Deep Learning

Deep neural networks have been shown to achieve state-of-the-art performance in several machine learning tasks. Stochastic Gradient Descent (SGD) is the preferred optimization algorithm for training these networks and asynchronous SGD (ASGD) has been widely adopted for accelerating the training of large-scale deep networks in a distributed computing environment. However, in practice it is quite challenging to tune the training hyperparameters (such as learning rate) when using ASGD so as achieve convergence and linear speedup, since the stability of the optimization algorithm is strongly influenced by the asynchronous nature of parameter updates. In this paper, we propose a variant of the ASGD algorithm in which the learning rate is modulated according to the gradient staleness and provide theoretical guarantees for convergence of this algorithm. Experimental verification is performed on commonly-used image classification benchmarks: CIFAR10 and Imagenet to demonstrate the superior effectiveness of the proposed approach, compared to SSGD (Synchronous SGD) and the conventional ASGD algorithm.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh latex
BIBTEX=bibtex
FIG2DEV=fig2dev

NAME=main
BIBNAME=iclr2016

all: $(NAME).pdf $(NAME).ps

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)
TEX=$(NAME).tex \
    $(BIBNAME).bib \

$(NAME).dvi: $(TEX) $(EPS) $(BIBNAME).bbl
	@echo Compiling $(NAME)
	@$(LATEX) $(NAME)
	@$(MAKE) fixlabels

$(NAME).pdf: $(NAME).dvi
	@dvipdfmx -p letter $(NAME).dvi

$(NAME).ps: $(NAME).dvi
	@dvips $(NAME).dvi
	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(NAME).log),0)
	@echo $(NAME) Compiling again to fix labels
	@$(LATEX) $(NAME)
else
	@echo $(NAME) Labels are correct
endif

$(BIBNAME).bbl: $(BIBNAME).bib
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(NAME)
	@echo Generating bibliography
	@$(BIBTEX) $(NAME)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(NAME)
	@$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(NAME).ps $(NAME).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf *.toc *.out *.bak


==> _region_.tex <==
\message{ !name(theory.tex)}
\message{ !name(theory.tex) !offset(14) }
\begin{eqnarray}
  g_i & = & \underbrace{\frac{1}{c}  \sum_{l = 1}^c \frac{\alpha_0}{\tau_{i,
  l}}  \underbrace{\left( \frac{1}{{\mu}}  \sum_{s = 1}^{{\mu}} \nabla
  f_{\xi_{i, s, l}} (\theta_{i - \tau_{i, l}}) \right)}_{\text{calculated in
  a learner}}}_{\text{aggregated in the parameter server}},  \label{dl-eq:1}\\
  \theta_{i + 1} & = & \underbrace{\theta_i - g_i}_{\text{calculated in the
                 parameter server}} , \nonumber
\end{eqnarray}
\message{ !name(theory.tex) !offset(-11) }


==> back.tex <==
\section{Background}
Distributed SGD is the primary method to solve deep learning problem. In any type of distributed SGD solver, there are two computation groups: parameter server group and learner group. Parameter server group hosts the model weights. Before each learner starts training, it pulls weights from the parameter server.  Each learner is responsible for sampling (a minibatch of) training data and calculating stochastic gradients based on sampled training data. Each learner sends its calculated stochastic gradients to the parameter server, while the server aggregates the gradients and applies weight update rules using aggregated gradients. 

There are two distributed SGD solving methods: Synchronous SGD (SSGD) and  Asynchronous SGD (ASGD). The key difference is that in SSGD each learner proceeds in lock-steps: Before each minibatch training, every learner pulls weights from the parameter server and every learner obtains the exactly same set of weights before it calculates the gradients. After the gradients are calculated by each learner, server aggregates gradients from each learner , each learner stalls until parameter server finishes applying gradient updates. In comparison, in ASGD, each learner trains neural network independent from other learners, there is no wait anywhere in learner.

ASGD has the obvious advantage that it runs much faster than SSGD. However, since each learner works on stale gradients with respect to each learner, the trained model might suffer significant accuracy loss. This paper proposes a solution to counter staleness in ASGD to minimize accuracy loss while achieving near linear speedup of runtime performance. \jltext{This section can be included in the introduction to show the difference between SSGD and ASGD. You can think a way to combine it with the introduction.}





==> hardsync.tex <==



==> meth_hook.tex <==
\subsection{Experimental Methodology}
\label{sec:meth_hook}
Please refer to Appendix~\ref{sec:meth} for the details of the hardware platform and the benchmarks used for experimental evaluation.


==> mulambda.tex <==
\section{Additional Finding}
In this Section, we demonstrate our  additional finding that when number of learners multiplies with minibatch size increases, the model accuracy decreases. 
\begin{table}
\vskip -0.1in
\centering
\small
    \begin{tabular}{cc|cc||c}

	\multicolumn{5}{c}{\CIFAR} \\
    \hline
               &    & \multicolumn{2}{c||}{Test error} & Time/epoch \\ 
    $\mu$ &  $\lambda$  & $\alpha_0 $ & $\alpha_0 / \tau$ & (sec)  \\ \hline
 \rowcolor{DarkGray}    128  &  1  & \multicolumn{2}{c||}{18.15\%}    & 148.15  \T \\ \hline
     			 128  &  30 &		NC		&		39.65\%	& 5.61 \T \\ 
	 			 64   &  30 &        NC		& 		31.18\% & 8.47  	\\
				 16   &  30 &        NC		& 		22.37\% & 10.28 	\\
\rowcolor{Gray} 	 4    &  30 &        NC		& 		17.92\% & 11.52 	\\
\rowcolor{Gray}	 2    &  60 &        NC		& 		18.21\% & 11.14 	\\	 	 	 
    \hline
    \end{tabular}
	\quad
	\quad
	 \begin{tabular}{cc|cc||c}
	\multicolumn{5}{c}{\imagenet} \\
    \hline     
    &  & \multicolumn{2}{c||}{Val. error} & Time/epoch \\ 
    $\mu$      &  $\lambda$         & $\alpha_0 $ & $\alpha_0 / \tau$ & (hrs)  \\
   \hline
\rowcolor{DarkGray}     256  &  1 & \multicolumn{2}{c||}{42.56\%}    & 49.83 \T \\ \hline
    				 256  &  18 &		NC		&		60.92\%	  & 2.83\T   \\ 
				 64   &  18 &       NC		& 		49.22\%   & 3.01 \\
	 			 32   &  18 &       NC		& 		46.55\%   & 3.33 \\
\rowcolor{Gray} 	 16   &  18 &       NC		& 		43.62\%   & 4.03 \\
\rowcolor{Gray}	 8    &  30 &       NC		& 		43.89\%   & 4.72 \\	 	 	 
    \hline
    \end{tabular}


   \caption{Test (top-1 validation) error on \CIFAR (\imagenet) on a model trained for 140 (35) epochs. NC = no convergence. $n$-softsync with $n=\lambda$ used in these experiments when $\lambda > 1$. Note that the column $\alpha=\alpha_0$ is equivalent to the Downpour-SGD}
  \label{tab:mullambda}
\end{table}

Table~\ref{tab:mullambda} lists the time/epoch and test error achieved on \CIFAR and \imagenet benchmarks for different configurations of $\mu$ and $\lambda$. 
In all cases, modulating the learning rate proves to be necessary in achieving convergence during distributed training of these models. 
As observed previously in Figure ~\ref{fig:speedup}, reducing $\mu$, the \minibatch size per learner, results in an increase in time/epoch. 
This is primarily due to the combined effect of degraded computational efficiency at each learner and more frequent communication between parameter servers and learners. 
Also note that in spite of using the staleness-dependent learning rate scheme, for a fixed number of learners $\lambda$, the test error increases monotonically with the \minibatch size $\mu$. 
%At the same time, configurations that keep the product $\mu\lambda$ constant yield similar test error when trained for the same number of epochs. 
At the same time, distributed training using ASGD and $\lambda$ learners can achieve model quality similar to SSGD (and within the same number of training epochs) so long as $\mu\lambda$ product is approximately the same as the \minibatch size used for SSGD.

These results help define a principled approach for distributed training of neural networks: \emph{the \minibatch size per learner should be reduced as more learners are added to the system in a way that keeps $\mu\lambda$ product constant. In addition, the learning rate should be modulated to account for stale gradients.}
These results reveal the scalability limits under the constraints of preserving the model accuracy. 
Since the smallest possible \minibatch size is 1, the maximum number of learners is bounded. 
This upper bound on the maximum number of learners can be relaxed if an inferior model is acceptable. 
Alternatively, it may be possible to reduce the test error for higher $\mu\lambda$ by training for a greater number of epochs. 
However, in such a scenario adding more learners to the system gives only a diminishing improvement in the overall training time. 
From machine learning and optimization perspective, this points to an interesting research direction that seeks to design optimization algorithm and learning strategies that perform well with large \minibatch sizes.

